Stochastic Subnetwork Annealing: A Regularization Technique for Fine Tuning Pruned Subnetworks

Pruning methods have recently grown in popularity as an effective way to reduce the size and computational complexity of deep neural networks. Large numbers of parameters can be removed from trained models with little discernible loss in accuracy after a small number of continued training epochs. However, pruning too many parameters at once often causes an initial steep drop in accuracy which can undermine convergence quality. Iterative pruning approaches mitigate this by gradually removing a small number of parameters over multiple epochs. However, this can still lead to subnetworks that overfit local regions of the loss landscape. We introduce a novel and effective approach to tuning subnetworks through a regularization technique we call Stochastic Subnetwork Annealing. Instead of removing parameters in a discrete manner, we instead represent subnetworks with stochastic masks where each parameter has a probabilistic chance of being included or excluded on any given forward pass. We anneal these probabilities over time such that subnetwork structure slowly evolves as mask values become more deterministic, allowing for a smoother and more robust optimization of subnetworks at high levels of sparsity.

==> notes.tex <==
dynamic partitiong.
 each weight guts a score which is prob distrivution of masking
 diff tasks diff partitions

==> outline.tex <==
introduction

Do this last?

related work

methods

neural partitioning. what happens if we partition a trained network into explicit independent subnetworks that share no hidden parameters?

algorithm: .....

parent network
creating the child networks
tuning the child networks
diversity aware loss function?
squishing all the child networks back into a single architecture (batch ensemble style)
making predictions

experiments

ablations
how many times can we split the parent network. what effect does parent size have on ensemble accuracy. bigger networks can accomodate more splits?

diversity
comparing the diversity of these partitions with other ensembles? partitions vs prune and tune.

comparison to other low-cost pseudo-ensembles
standard cifar stuff.

conclusions
